On the Long-term Impact of Algorithmic Decision Policies: Effort Unfairness and Feature Segregation through Social Learning

Most existing notions of algorithmic fairness are one-shot: they ensure some form of allocative equality at the time of decision making, but do not account for the adverse impact of the algorithmic decisions today on the long-term welfare and prosperity of certain segments of the population. We take a broader perspective on algorithmic fairness. We propose an effort-based measure of fairness and present a data-driven framework for characterizing the long-term impact of algorithmic policies on reshaping the underlying population. Motivated by the psychological literature on \emph{social learning} and the economic literature on equality of opportunity, we propose a micro-scale model of how individuals may respond to decision-making algorithms. We employ existing measures of segregation from sociology and economics to quantify the resulting macro-scale population-level change. Importantly, we observe that different models may shift the group-conditional distribution of qualifications in different directions. Our findings raise a number of important questions regarding the formalization of fairness for decision-making models.

==> experiments.tex <==
\section{Experiments}\label{sec:experiments}


\paragraph{The impact of benefit function}
TBD: False positives as role models---shifting the burden to decision maker as opposed to decision subjects.

==> impact.tex <==
\subsection{Measuring Impact through Segregation}\label{sec:impact}

Notable differences between our application domain and that of residential segregation are:
\begin{itemize}
\item Subjects (i.e. feature vectors) are often described by a multi-dimentional feature vectors---as opposed to 2-dimensional location in case of residential segregation. 
\item There is no predefined notion of ``area" or ``neighborhood" that individuals belong to. 
\item It is not immediately clear how distances and similarity between individuals should be defined. 
%\item \hh{Segregation is only undesirable when it works against the minority group's interest and well-being.}
\end{itemize}
Next, we will address these issues for the previously mentioned measures of segregation.

Throughout this section, we will focus on the mutable feature subspace.
We take the distance between two individuals $i$ (belonging to group $s$) and $j$ (belonging to group $s'$) as follows: $d(i,j) = \max\{d^s(i , j), d^{s'}(i , j)\}$, where $d^s(i , j)$ is defined as follows.
\begin{equation*}
\max\{ 0, q_s(y_j) - q_s(y_i) \} + \sum_{k \in \text{ muttable}} \epsilon_{s,k}(x_k,x'_k)
\end{equation*}
%\hh{We could alternatively define distance simply via the euclidean distance, but to ensure consistency, let's stick with the above.}

\paragraph{Evenness} We will use Atkinson index to measure evenness. We will specify areas through \emph{anchors} or \emph{focal points} (i.e. role models)---these are vectors that other subjects aspire to emulate in order to improve their utility. Each anchor corresponds to a neighborhood, and an individual belongs to the neighborhood of the nearest anchor.%An anchor is desirable if following it would improve the qualifications (true label).

\paragraph{Exposure} The SSI is independent of how areas are defined. For two individuals $i,j$, we will define $R_{i,j}$ (the intensity of connection between $i,j$) as follows:
$$R_{i,j} = c_{i,j} = e^{-d(i,j)} $$.
(Note that $B^s$ is a submatrix of $R$ constrained to rows and columns that correspond to members of group $s$).

%\paragraph{Concentration} is not of immediate interest in our application, so we will omit it entirely.%We first run a standard clustering algorithm to determine neighborhoods. We then compute the concentration index replacing area with volume.

\paragraph{Centralization} We measure the degree of centralization by comparing the percentage of minority individuals who are predicted to belong to a particular class/bucket (e.g. $\hY = 1$ or $\hY \in [0.5, 0.7]$).

\paragraph{Clustering} We will measure ACI at the individual level---that is, we assume each individual corresponds to a neighborhood. We will define $c_{i,j} = e^{-d(i,j)}$


Simulations to do:
\begin{itemize}
\item For each feature, look at its distribution before and after the change.
\item For different models, measure the above quantities before and after changes to the population. Illustrate the result in a bar plot.
\item Repeat the above, but this time focus on one model, but train it with two different sets of features, corresponding to immutable, and mutable attributes.
\end{itemize}




==> role_model_illustration.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t!]
\centering
\resizebox{0.5\columnwidth}{!}{
\tiny
\begin{tabular}{|c|c|c|}
\hline
% & \multicolumn{2}{  c |} {\bf Fairness} & {\bf Fairness} & \multicolumn{2}{ c |}{\bf Classifier Fairness} 
% \\ \cline{5-6}
{\bf Attribute} & {\bf Individual} & {\bf Role model} \\
\hline
\hline
%
Age & 27 & 33 \\
\hline
\rowcolor{lightgray}
Gender & Female & Female \\
\hline
\rowcolor{lightgray}
Marital status & Married & Married \\
\hline
Annual income & 100K & 80K \\
\hline
\rowcolor{YellowGreen}
Years employed & 1 year & 4 years \\
\hline
Annual spending & 60K & 60K \\
\hline
Income debt ratio & 0.3 & 0.9 \\
\hline
Recent late payments & 0 & 0 \\
\hline
\rowcolor{YellowGreen}
Length of credit history & 2 & 5 \\
\hline
Number of inquiries & 3 & 5 \\
\hline
\rowcolor{YellowGreen}
Co-applicant & No & Yes \\
\hline
\rowcolor{Yellow}
{\bf Monthly credit limit} & {\bf 5K} & {\bf 10K} \\
\hline
%
\end{tabular}
}
%\vspace{-2mm}
\caption{
    \small{
    A hypothetical example illustrating role model-based explanations. A customer demands to know why their credit limit is not high enough (e.g., 8K). We provide a contrastive explanation by showing them the characteristics of another customer who received high credit limit. The gray rows indicate immutable features. Green rows specify the qualifications of the role model the individual needs to match to get high credit limit.
    }
}
\label{fig:example}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> table.tex <==
 Table~\ref{tab:individual} shows the explanations offered to a male customer (individual 1) and a female customer (individual 2).


 Table~\ref{tab:group} shows the explanations offered to the group of male customers and the group of female customers.

==> user_exp_example.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[h!]
%\centering
%\resizebox{0.8\textwidth}{!}{
    \begin{tabular}{|p{5.9cm}|c|p{5.9cm}|c|c|}
\hline
% & \multicolumn{2}{  c |} {\bf Fairness} & {\bf Fairness} & \multicolumn{2}{ c |}{\bf Classifier Fairness} 
% \\ \cline{5-6}
{\bf \scriptsize Individual} & {\bf \scriptsize Model} & {\bf \scriptsize Explanation} & {\bf \scriptsize Effort} & {\bf \scriptsize Utility} \\
\hline
%
\multirow{4}{*}{\parbox{6cm}{
	{\scriptsize
    \begin{itemize}
    %\item $Y$ = True
    \item Gender = female
    \item MaxBillAmountOverLast6M = 3040
    \item MaxPaymentAmountOverLast6M = 1010
    \item MostRecentBillAmount = 1010
    \item TotalMonthsOverdue = 10
    \item TotalOverdueCounts = 2
    \end{itemize}
    }
    }}
& \scriptsize LogReg & \parbox{6cm}{
	{\scriptsize
    \begin{itemize}
    \item TotalMonthsOverdue = 4
    \end{itemize}}}
& \scriptsize 0.003 & \scriptsize 0.047 \\
\cline{2-5}
& \scriptsize DecTree & \parbox{6cm}{
	{\scriptsize
    \begin{itemize}
    \item TotalMonthsOverdue = 2
    \end{itemize}}}
& \scriptsize 0.004 & \scriptsize 0.046 \\
\cline{2-5}
& \scriptsize SVM & \parbox{6cm}{
	{\scriptsize
    \begin{itemize}
    \item TotalOverdueCounts = 1
    \end{itemize}}}
& \scriptsize 0.002 & \scriptsize 0.048 \\
\cline{2-5}
& \scriptsize NN & \parbox{6cm}{
	{\scriptsize
    \begin{itemize}
    \item MaxBillAmountOverLast6M = 850
    \item MaxPaymentAmountOverLast6M = 60
    \item MostRecentBillAmount = 830
    \item TotalMonthsOverdue = 3
    \end{itemize}
    }
    }
& \scriptsize 0.114 & \scriptsize -0.089 \\
\hline
%
%
\multirow{4}{*}{\parbox{6cm}{
	{\scriptsize
    \begin{itemize}
    %\item $Y$ = True
    \item Gender = male
    \item MWithHighSpendingOverLast6M = 0
    \item MaxBillAmountOverLast6M = 2290
    \item MostRecentBillAmount = 2160
    \item TotalMonthsOverdue = 10
    \item TotalOverdueCounts = 2
    \end{itemize}
    }
    }}
& \scriptsize LogReg & \parbox{6cm}{
	{\scriptsize
    \begin{itemize}
    \item TotalOverdueCounts = 1
    \end{itemize}}}
& \scriptsize 0.002 & \scriptsize 0.048 \\
\cline{2-5}
& \scriptsize DecTree & \parbox{6cm}{
	{\scriptsize
    \begin{itemize}
    \item MWithHighSpendingOverLast6M = 6
    \item MaxBillAmountOverLast6M = 980
    \item MostRecentBillAmount = 980
    \item TotalMonthsOverdue = 3
    \end{itemize}
    }
    }
& \scriptsize 0.087 & \scriptsize -0.062 \\
\cline{2-5}
& \scriptsize SVM & \parbox{6cm}{
	{\scriptsize
    \begin{itemize}
    \item MaxBillAmountOverLast6M = 620
    \item MostRecentBillAmount = 620
    \item TotalMonthsOverdue = 3
    \end{itemize}}}
& \scriptsize 0.068 & \scriptsize -0.043 \\
\cline{2-5}
& \scriptsize NN & \parbox{6cm}{
	{\scriptsize
    \begin{itemize}
    \item TotalMonthsOverdue = 1
    \end{itemize}}}
& \scriptsize 0.001 & \scriptsize 0.024 \\
\hline
%
\end{tabular}
%}
%\vspace{-2mm}
 \caption{
% 	\small{
        Example of the features and the explanations given to a female and male customer for four different classifiers together with the associated efforts and utilities.
        Both users are classified as defaulting in the next month by each of the models in spite of having a positive ground truth label.
        The customers receive explanations that differ in the features used and the suggested values because explanations for different classifiers use different role models.
        The two customers use different effort functions computed on their respective protected group.
 %   }
 }
 \label{fig:user_exp_example}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

